Correlative and Discriminative Label Grouping for Multi-Label Visual Prompt Tuning

Modeling label correlations has always played a pivotal role in multi-label image classification (MLC), attracting significant attention from researchers. However, recent studies have overemphasized co-occurrence relationships among labels, which can lead to overfitting risk on this overemphasis, resulting in suboptimal models. To tackle this problem, we advocate for balancing correlative and discriminative relationships among labels to mitigate the risk of overfitting and enhance model performance. To this end, we propose the Multi-Label Visual Prompt Tuning framework, a novel and parameter-efficient method that groups classes into multiple class subsets according to label co-occurrence and mutual exclusivity relationships, and then models them respectively to balance the two relationships. In this work, since each group contains multiple classes, multiple prompt tokens are adopted within Vision Transformer (ViT) to capture the correlation or discriminative label relationship within each group, and effectively learn correlation or discriminative representations for class subsets. On the other hand, each group contains multiple group-aware visual representations that may correspond to multiple classes, and the mixture of experts (MoE) model can cleverly assign them from the group-aware to the label-aware, adaptively obtaining label-aware representation, which is more conducive to classification. Experiments on multiple benchmark datasets show that our proposed approach achieves competitive results and outperforms SOTA methods on multiple pre-trained models.

==> sec/back_4_method.tex <==
\section{Method}
In this section, we describe a novel multi-label learning framework that exploits a class grouping strategy to learn both co- and dis-occurring representations, aimed at mitigating the adverse effects associated with co-occurrence relationships. 
In \S~\ref{sec:groupvpt}, we delineate the class grouping prompt tuning strategy to joint learning each class subset representation in co- and dis-occurring mode, respectively.
In \S~\ref{sec:moe_groupvpt}, to reflect the diversity of classes, we employ a Mixture-of-Expert model to assign distinct visual representations to each class, thereby obtaining a tailored visual representation for each class.
In the end, we describe in the \S~\ref{sec:optimization} how our co- and dis-occurring modes together to optimize and inference.

\paragraph{Overview of Our Method.} 
In an MLC task involving $K$ classes, we divide all classes into $N_c$ groups based on two distinct modes, namely co-occurrence and dis-occurrence modes, referred to as class subsets. Given a ViT backbone network, we freeze all its parameters and add a set of prompt tokens in co- and dis-occurrence mode, respectively. In each mode, these tokens are evenly distributed across several groups, with each group representing a class subset. Within the ViT framework, only extended prompt tokens need fine-tuning to effectively model both co- and dis-occurrence relationships among labels. Upon completing the modeling of label relationships, the ViT generates multiple visual representations for each class subset. 
\begin{align}
     \mathbf{Z}^{+} \cup \mathbf{Z}^{-} = {\rm ViT}_{\Phi}(\bm{x}),
\end{align}
Although these representations are shared among various classes within the same mode, the application of MoE allows for the derivation of distinct visual representations for each class across the two modes:
\begin{align}
     \mathbf{C}^{+} \!\!=\! {\rm MoE}\biguplus{\rm Gate}(\mathbf{Z}^{+})\text{,}~~\mathbf{C}^{-} \!\!=\! {\rm MoE}\biguplus{\rm Gate}(\mathbf{Z}^{-})\text{.}
\end{align}
where, $\biguplus$ indicates the weighted sum, MoE refers to the Mixture-of-Experts model, and Gate is the gating network.
Finally, we employ two sets of classifiers with non-shared parameters, each making predictions in their respective modes, and then combine the results using a weighted sum.
% 
\subsection{Co- and Dis- Occurrence Group Learning}\label{sec:groupvpt}
Modeling the correlations between labels has long been a key focus in MLL tasks~\cite{chen2019gcn,liu2021query2label}. However, overemphasizing these correlations often results in inferring objects primarily from co-occurring ones, which fails to capture all real-world scenarios~\cite{liu2022contextual}. On the other hand, learning discriminative representations for each object independently can lead to incorrect inferences when context or co-occurring objects are absent~\cite {wu2020adahgnn}. To address this issue, we decompose label correlation modeling into two aspects: In the co-occurrence mode, learning shared information for each class subset is utilized to model the relationships between co-occurring labels. Conversely, in the dis-occurrence mode, learning unique information for each class subset is employed to define the relationships between labels that do not co-occur.


Specifically, we divide the classes $\mathcal{C}$ into several smaller subsets within both co-occurrence and dis-occurrence modes, designated as $\{\mathcal{C}^{+}_{t}\}^{N_{c}}_{t=1}$ and $\{\mathcal{C}^{-}_{t}\}^{N_{c}}_{t=1}$, respectively, where $N_{c}$ is the number of subsets in each modes.
Additionally, the number of classes $|\mathcal{C}_{t}|$ within these subsets is expected to vary.
To implement the above grouping strategy, following previous work~\cite{chen2023boosting}, we construct a Co-occurrence Graph Partition (CGP), denoted as $\mathcal{G}^+$ and a Dis-occurrence Graph Partition (DGP), indicated as $\mathcal{G}^-$. The mathematical form can be written as follows:
\begin{align}
\bm{M}=
\begin{cases}
  \bm{M}^+= (\sqrt[\tau]{\bm{S}}+\sqrt[\tau]{\bm{S}}^\top)~/~{2},       & \mathcal{G}=\mathcal{G}^+ \\
  \bm{M}^-= \bm{I}-(\sqrt[\tau]{\bm{S}}+\sqrt[\tau]{\bm{S}}^\top)~/~{2}, & \mathcal{G}=\mathcal{G}^-
\end{cases}~\text{,}
\end{align}
where $\bm{M}$ is the association matrix of the class graph $\mathcal{G}$, and $\bm{S}$ denotes the label co-occurrence matrix~\cite{chen2019gcn}.
Subsequently, we apply spectral clustering to $\bm{M}$ in order to partition the classes $\mathcal{C}$ into smaller subsets, respectively:
\begin{align}
    \{\mathcal{C}^{+}_{t}\}^{N_{c}}_{t=1} \!\leftarrow\! {\rm cluster}(\bm{M}^+),\{\mathcal{C}^{-}_{t}\}^{N_{c}}_{t=1} \!\leftarrow\! {\rm cluster}(\bm{M}^-).
\end{align}
Here, {\rm cluster} refers to spectral clustering~\cite{von2007tutorial}.
%%%%%%%%%%%%%%%%%%%%
\subsection{Co- and Dis- Occurrence Group Learning}\label{sec:gvpt}
In MLL tasks, it is common to append a specific attention head to a visual encoder to decouple the image into multiple label-level visual representations~\cite{ye2020attention,liu2021query2label,ma2023semantic,chen2019iccv}, and will raise two primary concerns: {\textbf{\ding{182}}} During the feature extraction stage, the relationship between labels is not considered inside the visual encoder; {\textbf{\ding{183}}} The specific attention head overemphasizes the co-occurrence relationship, which brings the overfitting risk, as discussed in the \S \ref{sec:intro}.

Unlike the mainstream methods, our method emphasizes the importance of relationship modeling in learning visual representations. Moreover, to mitigate the overfitting risk associated with excessive label co-occurrence, we systematically assign all classes into co-occurrence groups and dis-occurrence groups, respectively.

Specifically, we define two types of prompt tokens, referred as to co-occurrence groups prompt $\{\mathbf{p}^{+}_{t}\}^{N_{c}}_{t=1}$ and co-occurrence groups prompt $\{\mathbf{p}^{-}_{t}\}^{N_{c}}_{t=1}$.
On the one hand, from the standpoint of grouping class, each prompt token $\mathbf{p}^{+}_{t}$ uniquely maps to a specific class subset $\mathcal{C}^{+}_{t}$. On the other hand, in terms of representation learning,  prompt token $\mathbf{p}^{+}_{t}$ is linked to all classes contained by $\mathcal{C}^{+}_{t}$, thereby forming a one-to-many relationship. 
For example, if $\mathcal{C}^{+}_{t}$ includes the classes {\ttfamily{\{bicycle;car;traffic light\}}}, then $\mathbf{p}^{+}_t$ is exclusively associated with these classes, which can indicate vision representations of these classes.
Similarly, the $\mathbf{p}^{-}_t$ corresponds directly to the $\mathcal{C}^{-}_{t}$.

In the context of visual prompt tuning, we introduce a set of co-occurrence group prompts $\mathbf{P}_{i-1}^{+} = \{\mathbf{p}_{i-1,t}^{+} \in \mathbb{R}^D | t \in \mathbb{N}, 1 \leq t \leq N_c\}$ and a set of dis-occurrence group prompts $\mathbf{P}_{i-1}^{-} = \{\mathbf{p}_{i-1,t}^{-} \in \mathbb{R}^D | t \in \mathbb{N}, 1 \leq t \leq N_c\}$ into each transformer block (${\rm Block}_{i}$), which is designed to facilitate the learning of visual representations pertinent to specific class subsets $\mathcal{C}^{+}_{t}$ and $\mathcal{C}^{-}_{t}$\footnote{The index $t$, in class subsets $\mathcal{C}_{t}^{+}$ and $\mathcal{C}_{t}^{-}$, may not be the same. However, for simplicity, we will uniformly denote it as $t$ in our analysis.}.
It is expressed in the following mathematical form:
\begin{align}\label{eq:group-vpt}
[\mathrm{cls}_{i},\!\mathbf{P}_{i}^{+},\!\mathbf{P}_{i}^{-},\!\mathbf{E}_{i}]\!=\!{\rm Block}_{i}([\mathrm{cls}_{i\!-\!1},\!\mathbf{P}_{i\!-\!1}^{+},\!\mathbf{P}_{i\!-\!1}^{-},\!\mathbf{E}_{i\!-\!1}]).
\end{align}
Leveraging the powerful long-range modeling advantages of the transformer block, each $\mathbf{p}_{i,t}$ can aggregate semantic information about the class subset $\mathcal{C}_{t}$ from the image embedding $\mathbf{E}_{i}$.
In the co-occurrence mode, $\mathbf{p}_{i,t}^{+}$ focuses on learning the shared semantic information within the category subset $\mathcal{C}_{t}^{+}$. Conversely, in the dis-occurrence mode, due to the significant semantic differences between the classes in subsets $\mathcal{C}_{t}^{-}$, the dis-occurrence group prompts $\mathbf{p}_{i,t}^{-}$ seeks to capture the distinct semantic information unique to each class within the subset.
However, due to the influence of the MSA, prompt tokens $\mathbf{p}_{i,t}$ may transfer information to one another. To mitigate this effect, we introduce a predefined mask (${\rm MASK}$) to prevent information exchange between prompt tokens, making them more discriminative.
After adding ${\rm MASK}$ to Eq. \eqref{eq:group-vpt}, it can be rewritten as follows:
\begin{equation}
\begin{aligned}
~ &  [\mathrm{cls}_{i}, \mathbf{P}_{i}^{+}, \mathbf{P}_{i}^{-}, \mathbf{E}_{i}] \\
=~ &  {\rm Block}_{i}([\mathrm{cls}_{i-1}, \mathbf{P}_{i-1}^{+}, \mathbf{P}_{i-1}^{-}, \mathbf{E}_{i-1}], {\rm MASK}).
\end{aligned}
\end{equation}
\subsection{More Prompt Token to Mixture-of-Experts}\label{sec:moe_groupvpt}
In the \S \ref{sec:gvpt}, each class subset was associated with a single prompt token. However, this simplification does not accurately represent the real-world scenarios, as each class exhibits diversity (\eg, color, shape, texture, etc.)~\cite{kwon2023probabilistic}, and multiple classes can concurrently share or possess distinct semantics. 
In the realm of category diversity research, drawing inspiration from prior studies~\cite{chen2023plot, kwon2023probabilistic}, we propose to implement a multi-prompt, that is,  a class subset $\mathcal{C}_{t}$ is linked to multiple prompts.

The above methods employ an optimization strategy (\eg, gaussian mixture models~\cite{kwon2023probabilistic}, optimal transport theory~\cite{villani2009optimal,chen2023plot}
) to address the selection challenges for multiple prompts to corresponding categories.
Nevertheless, our method offers a more direct solution that circumvents the dependence on ideal conditions within the optimization process. To be different from them, leveraging the benefits of MoE models in multi-task learning and enhancing model performance, we reformulate the selecting multi-prompt challenge into a multi-task learning problem.
% 
\paragraph{More Prompt Token.} Specifically, we extend each prompt token $\mathbf{p}_{i-1,t}$ from 1 to $N_{m}$, defined as follows: $\mathbf{p}_{i-1,t} = \{\mathbf{p}_{i-1,t}^{e} \in \mathbb{R}^D | e \in \mathbb{N}, 1 \leq e \leq N_m\}$.
Moreover, $\mathbf{p}_{i-1,t}^{e,+}$ indicates the co-occurrence group prompt tokens, while $\mathbf{p}_{i-1,t}^{e,-}$ is the dis-occurrence group prompt token.
To reduce the additional parameters, we advocate introducing MoE after the last transformer block.
Then, the final transformer block’s output can be expressed as: 
$[\mathrm{cls}_{o}, \mathbf{Z}^{+}, \mathbf{Z}^{-}, \mathbf{E}_{o}]$, where $\mathbf{Z}^{+}$ corresponds to the co-occurrence group output and $\mathbf{Z}^{-}$ corresponds to the dis-occurrence group output. More details, $\mathbf{z}_{t}^{e,-}$ is related to the $e$-th prompt token in the $t$-th co-occurrence group.
And, we refer to $\mathbf{z}_{t}^{e}$ as the $e$-th visual representation corresponding to the class subset $\mathcal{C}_{t}$.
% 
\paragraph{Mixture-of-Experts.} Subsequently, we introduce co-occurrence and dis-occurrence group experts $\mathcal{E}$, and each expert $E_{t}^{e}$ is implemented as an FFN with a ReLU activation and residual connection:
\begin{align}
    \mathcal{E}^{+} = \{ {E}_{t}^{e,+} | e, t \in \mathbb{N}, 1 \leq e \leq N_m, 1 \leq t \leq N_c\}~\text{,}\\
    \mathcal{E}^{-} = \{ {E}_{t}^{e,-} | e, t \in \mathbb{N}, 1 \leq e \leq N_m, 1 \leq t \leq N_c\}~\text{,}\\
    E_{t}^{e}(\mathbf{z}_{t}^{e}) = \mathbf{z}_{t}^{e} \!+\! \sigma(\mathbf{z}_{t}^{e} \mathbf{W}_{t,{\rm dn}}^{e} \!+\! \mathbf{b}_{t,{\rm dn}}^{e}) \mathbf{W}_{t,{\rm up}}^{e} \!+\! \mathbf{b}_{t,{\rm up}}^{e}~\text{,}
\end{align}
% where $\mathcal{E}$ indicates the set of experts, $E_{t}^{e}$ denote an expert, $\mathbf{W}_{t,{\rm dn}}^{e}$, $\mathbf{b}_{t,{\rm dn}}^{e}$, $\mathbf{W}_{t,{\rm up}}^{e}$, and $\mathbf{b}_{t,{\rm up}}^{e}$ are the weights and biases of the experts, and $\sigma$ is ReLU activation.
where $\mathbf{b}_{t,{\rm up}}^{e}$ are the weights and biases of the experts, and $\sigma$ is a ReLU activation.
To make lightweightness, the hidden dimension is kept small, \eg, set to 5. 
The two groups of experts don’t share parameters.
% \paragraph{Dynamic Gating Networks.}
\paragraph{Gating Networks.}
We employ two distinct strategies for expert selection: {\textbf{\ding{182}}} Each subset within the category group utilizes a dynamic routing network to learn varying weights for multiple representations $\mathbf{z}_{t}^{e}$, followed by weighted merging by multiple experts. {\textbf{\ding{183}}}
The second strategy considers each class independently; here, different classes within the corresponding class subset group employ different dynamic routing networks to determine diverse weights for multiple visual representations $\mathbf{z}_{t}^{e}$, subsequently merging these using multiple experts.
We opt for the second strategy, as different classes necessitate distinct information, rendering identical shared visual representations insufficient.

For each class $k$, we define a gating network $g_k(\cdot)$ in co- and dis-occurrence mode, respectively, implemented as a simple fully connected network:
\begin{align}
    \bm{w}_{k}^{+} &= {\rm Softmax}(\mathbf{z}_{t}^{e,+}\mathbf{W}_{k}^{+} + \mathbf{b}_{k}^{+} ) \in \mathrm{R}^{N_{m}}\text{,}~ k \in \mathcal{C}_{t}^{+}~\text{,} \\
    \bm{w}_{k}^{-} &= {\rm Softmax}(\mathbf{z}_{t}^{e,-}\mathbf{W}_{k}^{-} + \mathbf{b}_{k}^{+} ) \in \mathrm{R}^{N_{m}}\text{,}~ k \in \mathcal{C}_{t}^{-}~\text{,}
\end{align}
where $\bm{w}_{k}^{+} =\{w_{k}^{e,+}\}^{N_e}_{e=1}$ and $\bm{w}_{k}^{-} =\{w_{k}^{e,-}\}^{N_e}_{e=1}$ represent the gating weights associated with class $k$ in the class subset $\mathcal{C}^{+}_{t}$ and $\mathcal{C}^{-}_{t}$.
% 
\paragraph{Adaptive Aggregation Representation.}
Adaptively aggregate group representations into class-specific representations. The entire process of Mixture-of-Experts (MoE) is formalized as follows:
\begin{align}
     \mathbf{c}_{k}^{+} & = \sum\nolimits_{e=1}^{N_e} {w}_{k}^{e,+} E_{t}^{e,+}(\mathbf{z}_{t}^{e,+})~\text{,} \\
     \mathbf{c}_{k}^{-} & = \sum\nolimits_{e=1}^{N_e} {w}_{k}^{e,-} E_{t}^{e,-}(\mathbf{z}_{t}^{e,-})~\text{.}
\end{align}
where $\mathbf{c}_{k}^{+}$ and $\mathbf{c}_{k}^{-}$ indicate the visual representations for class $k$, obtained in the co-occurrence and dis-occurrence modes.
% 
\subsection{Optimization and Inference}\label{sec:optimization}
In this work, we adapt dual classification heads to mitigate the negative impacts arising from the accumulated prediction errors from a single classification head~\cite{xiecounterfactual}.
The predicted logits for both co- and dis-occurrence modes can be computed using a simple linear classifier as follows:
\begin{align}
    \hat{{y}}_{k}^{+} = {\rm Sigmoid}(\mathbf{W}_{k}^{\top}\mathbf{c}_{k,+}^{+} + {b}_{k}^{+})~,\\
    \hat{{y}}_{k}^{-} = {\rm Sigmoid}(\mathbf{W}_{k}^{\top}\mathbf{c}_{k,-}^{-} + {b}_{k}^{-})~.
\end{align}
Here, $\hat{{y}}_{k}^{+}$ and $\hat{{y}}_{k}^{-}$ represent the predictions for class $k$ in the two types of modes, while $f^{+}(\bm{x})= \hat{\bm{y}}^{+} =\{\hat{{y}}_{1}^{+}, \cdots, \hat{{y}}_{K}^{+} \}$ and $f^{-}(\bm{x}) = \hat{\bm{y}}^{-} =\{\hat{{y}}_{1}^{-}, \cdots, \hat{{y}}_{K}^{-} \}$ denote the predictions for all classes about instance $\bm{x}$, respectively.

Referring to Eq.~\eqref{eq:full-cls-expected-risk}, the overall expected risk associated with our proposed method can be reformulated as follows:
\begin{align}\label{eq:our-full-cls-expected-risk}
\mathcal{R}\left(f\right)=\mathbb{E}_{\left(\bm{x},\bm{y}\right)\sim p\left(\bm{x},\bm{y}\right)}\left[\mathcal{L}\left(f^{+}\left(\bm{x} \right), \bm{y} \right) + \mathcal{L}\left(f^{-}\left(\bm{x} \right), \bm{y} \right)
\right]~\text{.}
\end{align}

Given an instance $\bm{x}$, the model's final prediction is $f(\bm{x})= \hat{\bm{y}} = \hat{\bm{y}}^{+}+\hat{\bm{y}}^{-} = \{\hat{{y}}_{1}, \cdots, \hat{{y}}_{K} \}$.

==> table/coco_full.tex <==
\begin{table*}[htbp]
\setlength{\tabcolsep}{5pt}
\centering
\caption{MS-COCO}
\resizebox{\linewidth}{!}
{\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
\midrule
\midrule
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & 
\multicolumn{1}{c|}{\multirow{2}{*}{Backbone}} & 
\multicolumn{1}{c|}{\multirow{2}{*}{Pretrain}} &
\multicolumn{1}{c|}{\multirow{2}{*}{Resolution}} & 
\multicolumn{1}{c|}{\multirow{2}{*}{mAP}} & 
\multicolumn{6}{c|}{All}  & \multicolumn{6}{c|}{Top 3} &
\multicolumn{1}{c}{\multirow{2}{*}{lr}}  \\ 
\cline{6-17}
\multicolumn{1}{l|}{} &&&&&CP & CR & CF1 & OP & OR & 
OF1 & CP & CR & CF1 & OP & OR & OF1  \\
\midrule
\midrule
Linear & ResNet101 & ImageNet1k & 224$\times$224 & 68.8 &  64.1   &  64.7   &  64.4   &  67.8   &  68.6   &  68.2   & 60.1 & 59.1 & 59.6 & 61.4 & 63.4 & 62.4 & 0.0005\\

Linear & vit\_base\_patch16\_224 & ImageNet1k & 224$\times$224 & 71.6 &  66.7   &  67.2   &  66.9   &  69.3   &  70.1   &  69.7   & 61.0 & 61.8 & 61.4 & 62.4 & 64.4 & 63.4 & 0.0005\\

Linear & vit\_base\_patch16\_224\_in21k & ImageNet21k & 224$\times$224 & 70.9 &  65.9   &  66.5   &  66.2   &  69.3   &  70.0   &  69.7   & 60.4 & 60.7 & 60.6 & 62.2 & 64.3 & 63.2 & 0.0005\\

Linear & vit\_base\_mocov3 & ImageNet1k & 224$\times$224 & 67.0 &  62.8   &  63.3   &  63.1   &  67.4   &  68.2   &  67.8   & 59.2 & 57.5 & 58.3 & 60.8 & 62.8 & 61.8 & 0.0005\\

Linear & vit\_base\_patch16\_mae & ImageNet1k & 224$\times$224 & 53.1 &  52.0   &  52.5   &  52.2   &  59.9   &  60.6   &  60.2   & 49.6 & 48.1 & 48.9 & 55.3 & 57.1 & 56.2 & 0.0005\\

Linear & vit\_small\_dinov2 & LVD-142M & 224$\times$224 & 74.0 &  68.8   &  69.4   &  69.1   &  71.7   &  72.5   &  72.1   & 61.6 & 63.6 & 62.6 & 64.1 & 66.2 & 65.1 & 0.0005\\

Linear & vit\_base\_dinov2 & LVD-142M & 224$\times$224 & 78.2 &  72.6   &  73.2   &  72.9   &  74.4   &  75.2   &  74.8   & 65.8 & 66.7 & 66.3 & 66.2 & 68.3 & 67.2 & 0.0005\\
\midrule

VPT & vit\_base\_patch16\_224 & ImageNet1k & 224$\times$224 & 76.9 &  70.9   &  71.4   &  71.1   &  73.9   &  74.7   &  74.3   & 65.2 & 64.1 & 64.6 & 65.3 & 67.5 & 66.4 & 0.0005\\

VPT & vit\_base\_patch16\_224\_in21k & ImageNet21k & 224$\times$224 & 81.0 &  74.5   &  75.1   &  74.8   &  77.3   &  78.1   &  77.7   & 68.3 & 66.9 & 67.6 & 67.6 & 69.8 & 68.7 & 0.0005\\

VPT & vit\_base\_mocov3 & ImageNet1k & 224$\times$224 & 71.9 &  66.6   &  67.2   &  66.9   &  71.1   &  71.9   &  71.5   & 62.1 & 60.0 & 61.0 & 63.2 & 65.3 & 64.2 & 0.0005\\

VPT & vit\_base\_patch16\_mae & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT & vit\_small\_dinov2 & LVD-142M & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT & vit\_base\_dinov2 & LVD-142M & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\
\midrule

VPT+Group & vit\_base\_patch16\_224 & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group & vit\_base\_patch16\_224\_in21k & ImageNet21k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group & vit\_base\_mocov3 & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group & vit\_base\_patch16\_mae & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group & vit\_small\_dinov2 & LVD-142M & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group & vit\_base\_dinov2 & LVD-142M & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\
\midrule

VPT-30 & vit\_base\_patch16\_224 & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT-30 & vit\_base\_patch16\_224\_in21k & ImageNet21k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT-30 & vit\_base\_mocov3 & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT-30 & vit\_base\_patch16\_mae & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT-30 & vit\_small\_dinov2 & LVD-142M & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT-30 & vit\_base\_dinov2 & LVD-142M & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\
\midrule

VPT+Group+MoE-adapt & vit\_base\_patch16\_224 & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group+MoE-adapt & vit\_base\_patch16\_224\_in21k & ImageNet21k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group+MoE-adapt & vit\_base\_mocov3 & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group+MoE-adapt & vit\_base\_patch16\_mae & ImageNet1k & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group+MoE-adapt & vit\_small\_dinov2 & LVD-142M & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

VPT+Group+MoE-adapt & vit\_base\_dinov2 & LVD-142M & 224$\times$224 & - &  -   &  -   &  -   &  -   &  -   &  -   & - & - & - & - & - & - & 0.0005\\

\midrule
\midrule

\end{tabular}}
\vspace{0.1cm}
\label{Table:coco}
\end{table*}

% \multicolumn{1}{l|}{OF1}


% \rowcolor{gray!9} 
% \Xhline{5-8}{1.5pt}
% \cline{5-18}{\vrule width 1.5pt}
% \Xcline{5-18}{2pt}  % 加粗为 2pt
% \rowcolor{gray!9}
% \midrule
% \rowcolor{igray}
% \multirow{-1.8}{*}{\cellcolor{igray}Backbone} &  \cellcolor{igray}Prompt &  \cellcolor{igray}Group &  \cellcolor{igray}MoE &  mAP &  CP & CR & CF1 & OP & OR & OF1 &  mAP & CP & CR & CF1 & OP & OR & OF1 \\ 
% \midrule
% \Xcline{2pt}
% 
% \begin{table*}[hbt!]
% \begin{tabular}{c}
% \hline
% \noalign{\vskip -2pt}  % 调整线条位置
% \vrule height 2pt width \linewidth depth 0pt  % 自定义横线
% \noalign{\vskip 2pt}
% Data \\
% \hline
% \end{tabular}
% \end{table*}
% \begin{table*}
% \begin{tabular}{|>{\columncolor{gray!1}}c|>{\columncolor{gray!9}}c|>{\columncolor{gray!9}}c|}
% \hline
% \textbf{Header 1} & \textbf{Header 2} & \textbf{Header 3} \\ 
% \hline
% Data 1 & Data 2 & Data 3 \\
% \hline
% \end{tabular}
% \end{table*}
% \begin{table*}[hbt!]
% % \setlength{\tabcolsep}{5pt}
% % \setlength{\extrarowheight}{5pt} % 增加行高
% \centering
% \resizebox{\linewidth}{!}
% {\begin{tabular}{c|c c c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
% \hline\thickhline
% % \midrule
% % \rowcolor{igray}
% \multicolumn{1}{c|}{\cellcolor{igray}\multirow{2}{*}{Backbone}}  & 
% \multicolumn{3}{c|}{\cellcolor{igray}Scope} &
% % \cline{2-3}
% \multicolumn{7}{c|}{\cellcolor{igray}Resolution: 224 $\times$ 224} & \multicolumn{7}{c}{\cellcolor{igray}Resolution: 448 $\times$ 448} \\ 
% \cline{5-18}
% % \rowcolor{igray}
% \multicolumn{1}{l|}{\cellcolor{igray}} & \cellcolor{igray} Prompt & \cellcolor{igray} Group & \cellcolor{igray} MoE & \cellcolor{igray} mAP &  \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 & \cellcolor{igray} mAP & \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 \\ 
% \midrule
% \midrule
% ViT-B          & 1 & 2 &  3 &  4   &  5   &  6   &  7   &  8   &  9  & 10 &  11 &  12  & 13 & 14 & 15 & 16 & 17 \\
% % SRN               & 224$\times$224 & 77.1 & 81.6 & 65.4 & 71.2 & 82.7 & 69.9 & 75.8 & 85.2 & 58.8 & 67.4 & 87.4 & 62.5 & 72.9\\
% % ResNet-101        & 224$\times$224 & 78.3 & 80.2 & 66.7 & 72.8 & 83.9 & 70.8 & 76.8 & 84.1 & 59.4 & 69.7 & 89.1 & 62.8 & 73.6\\
% \midrule
% \end{tabular}}
% \vspace{0.1cm}
% \caption{Comparison of our method with known state-of-the-art models on MS-COCO at medium input resolution. The backbones noted with 22k are pretrained on the ImageNet-22k dataset.
% Among them, mAP, OF1, and CF1 are the primary metrics (shaded in the table) as the others may be affected by the chosen threshold largely. All metrics are in \%.}
% \label{Table:coco}
% \end{table*}
% \begin{table*}[h]
% \begin{tabular}{|c|c|}
% \hline
% \cellcolor{blue!25}\textcolor{white}{data1} & \cellcolor{blue!25}\textcolor{white}{data2} \\
% \hline
% data3 & data4 \\
% \hline
% \end{tabular}
% \end{table*}
% \setlength{\tabcolsep}{5pt}
% \setlength{\arrayrulewidth}{1.5pt}
% \setlength{\extrarowheight}{5pt} % 增加行高
% \begin{table*}[!t]
% \centering
% \caption{Comparison of our method with known state-of-the-art models on MS-COCO at medium input resolution. The backbones noted with 22k are pre-trained on the ImageNet-22k dataset.
% Among them, mAP, OF1, and CF1 are the primary metrics (shaded in the table) as the others may be affected by the chosen threshold largely. All metrics are in \%.}
% \resizebox{\linewidth}{!}
% {\begin{tabular}{c|c c c c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
% \hline\thickhline
% \multicolumn{1}{c|}{\multirow{2}{*}{\cellcolor{igray}}}
% & 
% \multicolumn{4}{c|}{\cellcolor{igray}Scope} &
% \multicolumn{7}{c|}{\cellcolor{igray}Resolution: 224 $\times$ 224} & \multicolumn{7}{c}{\cellcolor{igray}Resolution: 448 $\times$ 448} \\ 
% \cline{6-19}
% \multirow{-1.8}{*}{\cellcolor{igray}Backbone} &  \cellcolor{igray}GateVPT~\cite{yoo2023improving} & \cellcolor{igray}VPT~\cite{jia2022visual} &  \cellcolor{igray}Group &  \cellcolor{igray}MoE &  \cellcolor{igray}mAP &  \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 &  \cellcolor{igray}mAP & \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 \\ 
% \hline
% \midrule
% ViT-B         & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% ViT-B         &            & \checkmark &            &            & 76.9 & 70.9 & 71.4 & 71.1 & 73.9 & 74.7 & 74.3 & - & - & - & -  & - & - & - \\
% ViT-B         &            &            & \checkmark &            & 78.4 & 72.0 & 72.6 & 72.3 & 75.0 & 75.7 & 75.3 & - & - & - & -  & - & - & - \\
% ViT-B         &            &            & \checkmark & \checkmark & 79.3 & 72.8 & 73.4 & 73.1 & 75.6 & 76.4 & 76.0 & - & - & - & -  & - & - & - \\
% \midrule
% MEA              & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% MEA              &            & \checkmark &            &            & 68.2 & 63.9 & 64.4 & 64.2 & 69.6 & 70.3 & 70.0 & - & - & - & -  & - & - & - \\
% MEA              &            &            & \checkmark &            & 71.2 & 66.1 & 66.6 & 66.4 & 71.5 & 72.3 & 71.9 & - & - & - & -  & - & - & - \\
% MEA              &            &            & \checkmark & \checkmark & 74.6 & 68.8 & 69.4 & 69.1 & 73.5 & 74.3 & 73.9 & - & - & - & -  & - & - & - \\
% \midrule
% MoCo v3           & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% MoCo v3           &            & \checkmark &            &            & 71.9 & 66.6 & 67.2 & 66.9 & 71.1 & 71.9 & 71.5 & - & - & - & -  & - & - & - \\
% MoCo v3           &            &            & \checkmark &            & 72.9 & 67.5 & 68.0 & 67.8 & 71.8 & 72.6 & 72.2 & - & - & - & -  & - & - & - \\
% MoCo v3           &            &            & \checkmark & \checkmark & 74.4 & 68.8 & 69.3 & 69.0 & 72.9 & 73.6 & 73.2 & - & - & - & -  & - & - & - \\
% \midrule
% ViT-B-21k     & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% ViT-B-21k     &            & \checkmark &            &            & 81.0 & 74.5 & 75.1 & 74.8 & 77.3 & 78.1 & 77.7 & - & - & - & -  & - & - & - \\
% ViT-B-21k     &            &            & \checkmark &            & 82.1 & 75.5 & 76.0 & 75.7 & 77.9 & 78.8 & 78.4 & - & - & - & -  & - & - & - \\
% ViT-B-21k     &            &            & \checkmark & \checkmark & 82.9 & 76.0 & 76.6 & 76.3 & 78.5 & 79.4 & 78.9 & - & - & - & -  & - & - & - \\
% \midrule
% DINOv2/B         & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% DINOv2/B         &            & \checkmark &            &            & 86.1 & 79.5 & 80.1 & 79.8 & 81.9 & 82.8 & 82.4 & - & - & - & -  & - & - & - \\
% DINOv2/B         &            &            & \checkmark &            & 87.0 & 80.3 & 80.9 & 80.6 & 82.7 & 83.5 & 83.1 & - & - & - & -  & - & - & - \\
% DINOv2/B         &            &            & \checkmark & \checkmark & 87.4 & 80.6 & 81.2 & 80.9 & 82.9 & 83.8 & 83.4 & - & - & - & -  & - & - & - \\
% \midrule
% DINOv2/S         & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% DINOv2/S         &            & \checkmark &            &            & 80.1 & 73.8 & 74.4 & 74.1 & 77.1 & 77.9 & 77.5 & - & - & - & -  & - & - & - \\
% DINOv2/S         &            &            & \checkmark &            & 81.5 & 74.9 & 75.5 & 75.2 & 78.2 & 79.1 & 78.6 & - & - & - & - & - & - & - \\
% DINOv2/S         &            &            & \checkmark & \checkmark & 82.9 & 76.2 & 76.8 & 76.5 & 79.2 & 80.0 & 79.6 & - & - & - & -  & - & - & - \\
% \bottomrule
% \end{tabular}}
% \label{Table:coco}
% \end{table*}

==> table/nus_vg256_in_app.tex <==
\begin{table*}[!t]
% \renewcommand\arraystretch{0.75}
\centering
\caption{Comparison of our method with state-of-the-art models on NUS-WIDE and VG256 at 224 resolution. All metrics are in \%.}
\vspace{-1.0em}
\resizebox{1.0\linewidth}{!}
{\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
\hline\thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\cellcolor{igray}}}
&
\multicolumn{1}{c|}{\multirow{2}{*}{\cellcolor{igray}}}
& 
\multicolumn{7}{c|}{\cellcolor{igray}NUS} & \multicolumn{7}{c}{\cellcolor{igray}VG256} \\ 
% \cline{6-19}
\multirow{-1.8}{*}{\cellcolor{igray}Method} & \multirow{-1.8}{*}{\cellcolor{igray}Backbone} &   \cellcolor{igray}mAP &  \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 &  \cellcolor{igray}mAP & \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 \\ 
\hline
\midrule
VPT      & ViT-B        & 65.2 & 62.9 & 62.7 & 62.8 & 74.0 & 73.7 & 73.8 & 42.2 & 43.8 & 44.2 & 44.0 & 57.4 & 57.6 & 57.5  \\
GateVPT  & ViT-B        & 62.8 & 61.6 & 61.4 & 61.5 & 73.0 & 72.8 & 72.9 & 41.1 & 42.9 & 43.2 & 43.0 & 56.4 & 56.6 & 56.5  \\
E2VPT    & ViT-B        & 63.9 & 62.4 & 62.1 & 62.2 & 73.8 & 73.6 & 73.7 & 42.2 & 44.0 & 44.3 & 44.2 & 57.5 & 57.7 & 57.6  \\ 
Ours     & ViT-B        & 65.7 & 63.4 & 63.2 & 63.3 & 74.3 & 74.0 & 74.1 & 44.2 & 45.6 & 45.9 & 45.8 & 58.8 & 58.9 & 58.8  \\
\midrule
VPT      & MAE          & 60.3 & 59.4 & 59.2 & 59.3 & 73.1 & 72.9 & 73.0 & 37.9 & 40.2 & 40.5 & 40.3 & 55.1 & 55.3 & 55.2  \\
GateVPT  & MAE          & 58.2 & 57.7 & 57.5 & 57.6 & 72.0 & 71.7 & 71.9 & 35.3 & 38.1 & 38.3 & 38.2 & 53.1 & 53.3 & 53.2  \\
E2VPT    & MAE          & 60.6 & 59.5 & 59.3 & 59.4 & 73.1 & 72.9 & 73.0 & 37.6 & 40.1 & 40.3 & 40.2 & 54.9 & 55.1 & 55.0  \\
Ours     & MAE          & 61.9 & 60.8 & 60.5 & 60.7 & 73.6 & 73.3 & 73.5 & 40.5 & 42.5 & 42.8 & 42.7 & 57.2 & 57.4 & 57.3  \\
\midrule
VPT      & MoCo v3      & 62.7 & 61.4 & 61.2 & 61.3 & 73.6 & 73.4 & 73.8 & 40.4 & 42.5 & 42.8 & 42.6 & 56.4 & 56.6 & 56.5  \\
GateVPT  & MoCo v3      & 61.8 & 60.6 & 60.4 & 60.5 & 73.0 & 72.7 & 72.9 & 39.6 & 41.7 & 42.0 & 41.8 & 55.7 & 55.9 & 55.8  \\
E2VPT    & MoCo v3      & 62.8 & 61.3 & 61.0 & 61.2 & 73.6 & 73.4 & 73.5 & 40.4 & 42.3 & 42.6 & 42.5 & 56.4 & 56.6 & 56.5  \\
Ours     & MoCo v3      & 63.0 & 61.2 & 60.9 & 61.1 & 73.8 & 73.5 & 73.6 & 41.0 & 43.0 & 43.2 & 43.1 & 57.0 & 57.1 & 57.1  \\
\midrule
VPT      & ViT-B-21k    & 67.5 & 65.0 & 64.7 & 64.8 & 74.8 & 74.6 & 74.7 & 46.0 & 47.2 & 47.6 & 47.4 & 60.1 & 60.3 & 60.2  \\
GateVPT  & ViT-B-21k    & 66.9 & 64.6 & 64.3 & 64.4 & 74.4 & 74.2 & 74.3 & 45.4 & 46.6 & 47.0 & 46.8 & 59.4 & 59.6 & 59.5  \\
E2VPT    & ViT-B-21k    & 67.7 & 65.1 & 64.8 & 64.9 & 74.9 & 74.6 & 74.7 & 46.0 & 47.3 & 47.6 & 47.4 & 60.0 & 60.2 & 60.1  \\
Ours     & ViT-B-21k    & 68.2 & 65.2 & 64.9 & 65.0 & 75.2 & 74.9 & 75.0 & 47.6 & 48.5 & 48.8 & 48.6 & 61.1 & 61.3 & 61.2  \\
\midrule
VPT      & DINOv2/B     & 68.1 & 65.3 & 65.0 & 65.1 & 75.1 & 74.8 & 75.0 & 49.3 & 50.1 & 50.5 & 50.3 & 62.8 & 63.0 & 62.9  \\
GateVPT  & DINOv2/B     & 67.2 & 64.7 & 64.5 & 64.6 & 74.6 & 74.4 & 74.5 & 48.6 & 49.5 & 49.9 & 49.7 & 62.3 & 62.5 & 62.4  \\
E2VPT    & DINOv2/B     & 67.9 & 65.1 & 64.8 & 65.0 & 75.1 & 74.8 & 75.0 & 49.2 & 50.1 & 50.5 & 50.3 & 62.8 & 63.0 & 62.9  \\
Ours     & DINOv2/B     & 68.7 & 65.6 & 65.3 & 65.5 & 75.3 & 75.0 & 75.2 & 50.9 & 51.6 & 51.9 & 51.7 & 64.0 & 64.2 & 64.1  \\
\midrule
VPT      & DINOv2/S     & 65.3 & 63.3 & 63.1 & 63.2 & 74.4 & 74.2 & 74.3 & 45.2 & 46.6 & 46.9 & 46.7 & 60.1 & 60.3 & 60.2  \\
GateVPT  & DINOv2/S     & 64.5 & 62.7 & 62.4 & 62.6 & 73.8 & 73.6 & 73.7 & 44.3 & 45.7 & 46.0 & 45.9 & 59.2 & 59.4 & 59.3  \\
E2VPT    & DINOv2/S     & 65.4 & 63.2 & 63.0 & 63.1 & 74.4 & 74.1 & 74.3 & 45.1 & 46.5 & 46.8 & 46.7 & 60.0 & 60.2 & 60.1  \\
Ours     & DINOv2/S     & 66.9 & 64.5 & 64.1 & 64.3 & 74.9 & 74.6 & 74.8 & 47.7 & 48.5 & 48.8 & 48.7 & 61.8 & 62.0 & 61.9  \\
\bottomrule
\end{tabular}}
\label{app_tab:nusvg256}
\end{table*}


% 45.2 & 46.6 & 46.9 & 46.7 & 60.1 & 60.3 & 60.2 
% 44.3 & 45.7 & 46.0 & 45.9 & 59.2 & 59.4 & 59.3 
% 45.1 & 46.5 & 46.8 & 46.7 & 60.0 & 60.2 & 60.1 
% 47.7 & 48.5 & 48.8 & 48.7 & 61.8 & 62.0 & 61.9 

==> table/sota_coco.tex <==
\begin{table*}[!t]
\centering
\caption{Comparison results on MS-COCO between our method and SOTA methods. All metrics are in \%.}
\begin{tabular}{l | c | c | c | c | c | c | c | c | c | c}
    \midrule\midrule
    Method             & Backbone     & Pre-trained Data  & Resolution      & mAP  & CP   & CR   & CF1  & OP   & OR & OF1 \\
    \midrule
    % SRN                & ResNet101      & $224\times 224$ & 77.1 & 81.6 & 65.4 & 71.2 & 82.7 & 69.9 & 75.8              \\
    % ResNet-101         & ResNet101      & $224\times 224$ & 78.3 & 80.2 & 66.7 & 72.8 & 83.9 & 70.8 & 76.8              \\
    % CADM               & ResNet101      & $448\times 448$ & 82.3 & 82.5 & 72.2 & 77.0 & 84.0 & 75.6 & 79.6              \\
    ML-GCN             & ResNet101    & ImageNet 1K       & $448\times 448$ & 83.0 & 85.1 & 72.0 & 78.0 & 85.8 & 75.4 & 80.3              \\
    % KSSNet             & ResNet101      & $448\times 448$ & 83.7 & 84.6 & 73.2 & 77.2 & 87.8 & 76.2 & 81.5              \\
    % MS-CMA             & ResNet101      & $448\times 448$ & 83.8 & 82.9 & 74.4 & 78.4 & 84.4 & 77.9 & 81.0              \\
    % MCAR               & ResNet101      & $448\times 448$ & 83.8 & 85.0 & 72.1 & 78.0 & 88.0 & 73.9 & 80.3              \\
    % CPSD               & ResNet101      & $448\times 448$ & 83.1 & 83.5 & 73.6 & 78.2 & 84.8 & 77.3 & 80.9              \\
    IDA                & ResNet101    & ImageNet 1K       & $448\times 448$ & 84.8 & -    & -    & 78.7 & -    & -    & 80.9              \\
    SSGRL              & ResNet101    & ImageNet 1K       & $576\times 576$ & 83.8 & 89.9 & 68.5 & 76.8 & 91.3 & 70.8 & 79.7              \\
    Q2L-R101           & ResNet101    & ImageNet 1K       & $448\times 448$ &  84.9& 84.8 &74.5  &79.3  & 86.6 & 76.9 & 81.5              \\
    C-Trans            & ResNet101    & ImageNet 1K       & $576\times 576$ & 85.1 & 86.3 & 74.3 & 79.9 & 87.7 & 76.5 & 81.7              \\
    ADD-GCN            & ResNet101    & ImageNet 1K       & $576\times 576$ & 85.2 & 84.7 & 75.9 & 80.1 & 84.9 & 79.4 & 82.0              \\
    % \midrule 
    % PAT-T              & ResNet101      & $448\times 448$ & 85.0 & 87.6 & 74.4 & 80.5 & 88.4 &	77.9 & 82.8 \\ 
    \midrule
    ASL                & TResNetL     & ImageNet 1K       & $448\times 448$ & 86.6 & 87.2 & 76.4 & 81.4 & 88.2 & 79.2 & 81.8             \\
    CPSD               & TResNetL     & ImageNet 1K       & $448\times 448$ & 87.3 & 85.5 & 78.9 & 82.1 & 85.7 & 81.5 & 83.7             \\
    Q2L-TResL          & TResNetL     & ImageNet 1K       & $448\times 448$ & 87.3 & 87.6 & 76.5 & 81.6 & 88.4 & 78.5 & 83.1             \\
    Q2L-TResL          & TResNetL-21K & ImageNet 21K      & $448\times 448$ & 89.2 & 86.3 & 81.4 & 83.8 & 86.5 & 83.3 & 84.9             \\
    \midrule
    M3TR               & ViT-B-21K    & ImageNet 21K      & $448\times 448$ & 87.5 & 88.4 & 77.2 & 82.5 & 88.3 & 79.8 & 83.8             \\
    PatchCT            & ViT-B-21K    & ImageNet 21K      & $448\times 448$ & 88.3 & 83.3 & 82.3 & 82.6 & 84.2 & 83.7 & 83.8             \\
    \midrule
    ML-VPT (Ours)      & DINOv2       & LVD-142M          & $448\times 448$ & \cellcolor{igray2}90.6 & 84.2 & 84.8 & \cellcolor{igray2}84.5 & 86.0 & 86.9 & \cellcolor{igray2}86.4             \\
    % TResNetL           & TResNetL (21k) & $448\times 448$ & 88.4 & -    &  -   & -    & -    &  -   & -                \\
    \midrule\midrule
%		TResNetL & TResNetL (OI)         & 71.01          & 72.98          & 74.49          & 53.60           & 57.06          & 58.53          & 59.24          \\
    % \midrule
    % PAT-T              & TResNetL       & $448\times 448$ & 88.7 & 89.0 & 78.8 & 83.6 &	89.3 &	81.3 & 85.1 
    % \\
    % PAT-T              & TResNetL (21k) & $448\times 448$ & 90.6 & 90.6 & 81.0 & 85.5 &	90.9 &	82.9 & 86.7 
    % \\
%		PAT-T      & TResNetL (OI)        & 71.01          & 72.98          & 74.49          & 53.60           & 57.06          & 58.53          & 59.24          \\
    % \midrule
    % Q2L-TResL          & TResNetL       & $448\times 448$ & 87.3 & 87.6 & 76.5 & 81.6 & 88.4 & 78.5 & 83.1 \\
    % Q2L-TResL          & TResNetL (21k) & $448\times 448$ & 89.2 & 86.3 & 81.4 & 83.8 & 86.5 & 83.3 & 84.9 \\
    %		Q2L-TResL      & TResNet (OI)        & 71.01          & 72.98          & 74.49          & 53.60           & 57.06          & 58.53          & 59.24          \\
		%		ML-Decoder      & TResNet (OI)        & 71.01          & 72.98          & 74.49          & 53.60           & 57.06          & 58.53          & 59.24          \\
    % \midrule
    % PAT-T + Q2L-TResL  & TResNetL       & $448\times 448$ & 89.5 & 89.5 & 79.3 &	84.1 & 90.0 & 81.0 & 85.3  \\
    % PAT-T + Q2L-TResL  & TResNetL (21k) & $448\times 448$ & 91.0 & 89.1 & 82.7 &	85.8 &	89.8& 	83.9 &	86.8 
    % \\
    % \midrule
    % ML-Dec             & TResNetL (OI)   & $448\times 448$ & 90.0 & -    & -    & -     & -     &   -   & -    \\ 
    % Q2L-TResL          & TResNetL (OI)   & $448\times 448$ & 90.1 & 83.6 &	84.2 & 	83.9 & 	85.0 & 	85.9 &	85.4 
    % \\ 
    % Q2L-SwinL          & Swin-L(21k)     & $384\times 384$ & 90.5 & 89.4 & 81.7 & 85.4 & 89.8 & 83.2 & 86.4 \\ 
    % Q2L-CvT            & CvT-w24(21k)    & $448\times 448$ & 91.3 & 88.8 & 83.2 & 85.9 & 89.2 & 84.6 & 86.8 \\
    % \midrule
    % PAT-T + ML-Dec     & TResNetL (OI)   & $448\times 448$ & 91.4 & 90.1 & 82.9 & \textbf{86.4}  & 90.5 & 84.8 & \textbf{87.6}  \\
    % PAT-T + Q2L-TResL  & TResNetL (OI)   & $448\times 448$ & \textbf{91.7} & 89.7 & 83.4 & \textbf{86.4} & 90.3 & 84.9 & 87.5   \\
    \end{tabular}
    \label{tab:sotacoco}
\end{table*}

==> table/voc_in_app.tex <==
\begin{table*}[!t]
\renewcommand\arraystretch{0.55}
\centering
\caption{Comparison of our method with state-of-the-art models on VOC2007 at 224 and 448 resolution. All metrics are in \%.}
\vspace{-1.0em}
\resizebox{0.95\linewidth}{!}
{\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
\hline\thickhline
\multicolumn{1}{c|}{\multirow{2}{*}{\cellcolor{igray}}}
&
\multicolumn{1}{c|}{\multirow{2}{*}{\cellcolor{igray}}}
& 
\multicolumn{7}{c|}{\cellcolor{igray}Resolution: 224 $\times$ 224} & \multicolumn{7}{c}{\cellcolor{igray}Resolution: 448 $\times$ 448} \\ 
% \cline{6-19}
\multirow{-1.8}{*}{\cellcolor{igray}Method} & \multirow{-1.8}{*}{\cellcolor{igray}Backbone} &   \cellcolor{igray}mAP &  \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 &  \cellcolor{igray}mAP & \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 \\
\hline
\midrule
VPT      & ViT-B     & 90.4 & 81.6 & 85.3 & 83.4 & 84.5 & 86.9 & 85.7 & 93.4 & 85.4 & 89.4 & 87.4 & 87.9 & 90.4 & 89.1 \\
GateVPT  & ViT-B     & 87.4 & 79.1 & 82.7 & 80.9 & 81.7 & 84.1 & 82.9 & 89.2 & 81.3 & 85.0 & 83.1  & 84.0 & 86.4 & 85.2 \\
E2VPT    & ViT-B     & 85.8 & 77.6 & 81.3 & 79.4 & 82.6 & 84.9 & 83.7 & 92.4 & 84.6 & 88.5 & 86.5 & 87.1 & 89.6 & 88.3  \\
% vpt-group& ViT-B & 78.4 & 72.0 & 72.6 & 72.3 & 75.0 & 75.7 & 75.3 & - & - & - & -  & - & - & - \\
Ours     & ViT-B     & 92.9 & 84.5 & 88.4 & 86.4 & 86.9 & 89.4 & 88.1 & 94.3 & 86.6 & 90.6 & 88.6 & 88.9 & 91.4 & 90.1 \\
\midrule
VPT      & MAE          & 80.3 & 72.5 & 75.8 & 74.1 & 79.1 & 80.4 & 79.2 & 82.8 & 74.3 & 77.6 & 75.9 & 80.5 & 82.8 & 81.6  \\
GateVPT  & MAE          & 85.1 & 73.6 & 77.3 & 75.4 & 79.3 & 81.8 & 80.5 & 86.1 & 77.5 & 81.0 & 79.2 & 83.0 & 85.4 & 84.2  \\
E2VPT    & MAE          & 83.3 & 75.0 & 78.5 & 76.7 & 80.3 & 82.6 & 81.5 & 84.6 & 76.5 & 80.0 & 78.2 & 82.0 & 84.4 & 83.2  \\
% vpt-group & MEA & 71.2 & 66.1 & 66.6 & 66.4 & 71.5 & 72.3 & 71.9 & - & - & - & -  & - & - & -\\
Ours     & MAE          & 88.8 & 80.2 & 83.9 & 82.0 & 84.7 & 87.1 & 85.9 & 90.4 & 82.1 & 85.9 & 83.9 & 86.2 & 88.7 & 87.4 \\
\midrule
VPT      & MoCo v3       & 86.2 & 78.0 & 81.6 & 79.7 & 82.4 & 84.8 & 83.6 & 88.4 & 80.5 & 84.2 & 82.3 & 84.5 & 86.9 & 85.7  \\ 
GateVPT  & MoCo v3       & 83.5 & 75.4 & 78.9 & 77.1 & 80.0 & 82.4 & 81.2 & 87.7 & 79.3 & 83.0 & 81.1 & 83.5 & 85.9 & 84.7  \\
E2VPT    & MoCo v3       & 85.9 & 77.5 & 81.0 & 79.2 & 81.9 & 84.3 & 83.1 & 88.8 & 80.5 & 84.3 & 82.4 & 84.4 & 86.9 & 85.6  \\
% vpt-group& MoCo v3 & 72.9 & 67.5 & 68.0 & 67.8 & 71.8 & 72.6 & 72.2 & - & - & - & -  & - & - & -\\
Ours     & MoCo v3       & 91.1 & 82.3 & 86.1 & 84.2 & 85.6 & 88.0 & 86.8 & 92.7 & 84.4 & 88.2 & 86.3 & 87.4 & 89.8 & 88.6  \\
\midrule
VPT      & ViT-B-21k & 94.2 & 86.0 & 90.0 & 88.0 & 88.3 & 90.8 & 89.6 & 94.4 & 86.7 & 90.7 & 88.7 & 89.2 & 91.7 & 90.4 \\
GateVPT  & ViT-B-21k & 94.3 & 96.5 & 90.6 & 88.5 & 88.5 & 91.0 & 89.7 & 95.2 & 87.6 & 91.6 & 89.6  & 89.9 & 92.4 & 91.1 \\
E2VPT    & ViT-B-21k & 94.1 & 86.0 & 89.9 & 87.9 & 88.2 & 90.7 & 89.4 & 95.1 & 87.3 & 91.4 & 89.3 & 89.5 & 92.0 & 90.7 \\
% vpt-group & ViT-B-21k & 82.1 & 75.5 & 76.0 & 75.7 & 77.9 & 78.8 & 78.4 & - & - & - & -  & - & - & - \\
Ours     & ViT-B-21k & 94.7 & 86.9 & 90.9 & 88.8 & 88.9 & 91.4 & 90.1 & 95.6 & 88.0 & 92.1 & 90.0 & 90.1 & 92.6 & 91.3  \\
\midrule
VPT      & DINOv2/B    & 95.6 & 88.2 & 92.3 & 90.2 & 90.3 & 92.9 & 91.6 & 96.1 & 89.0 & 93.1 & 91.0 & 91.0 & 93.6 & 92.3 \\
GateVPT  & DINOv2/B    & 95.5 & 87.7 & 91.7 & 89.7 & 90.0 & 92.5 & 91.2 & 96.2 & 89.0 & 93.2 & 91.1  & 91.2 & 93.8 & 92.5 \\
E2VPT    & DINOv2/B    & 95.4 & 87.9 & 92.0 & 89.9 & 90.2 & 92.7 & 91.4 & 96.1 & 89.1 & 93.2 & 91.1 & 91.1 & 93.7 & 92.4 \\
% vpt-group& DINOv2/B & 87.0 & 80.3 & 80.9 & 80.6 & 82.7 & 83.5 & 83.1 & - & - & - & -  & - & - & - \\
Ours     & DINOv2/B    & 96.4 & 88.9 & 93.0 & 90.9 & 90.9 & 93.5 & 92.2 & 97.0 & 90.0 & 94.2 & 92.1 & 91.9 & 94.4 & 93.1 \\
\midrule
VPT      & DINOv2/S    & 92.8 & 84.5 & 88.4 & 86.4 & 87.3 & 89.8 & 88.5 & 93.8 & 86.1 & 90.1 & 88.1 & 88.9 & 91.4 & 90.1  \\
GateVPT  & DINOv2/S    & 92.1 & 83.6 & 87.5 & 85.5 & 86.5 & 88.9 & 87.7 & 93.3 & 85.3 & 89.3 & 87.3  & 88.1 & 90.6 & 89.3 \\
E2VPT    & DINOv2/S    & 89.6 & 81.3 & 85.0 & 83.1 & 85.2 & 87.6 & 86.3 & 91.2 & 83.0 & 86.8 & 84.8 & 86.7 & 89.3 & 88.0 \\
% vpt-group& DINOv2/S  & 81.5 & 74.9 & 75.5 & 75.2 & 78.2 & 79.1 & 78.6 & - & - & - & - & - & - & -\\
Ours     & DINOv2/S    & 94.2 & 86.4 & 90.3 & 88.3 & 89.0 & 91.5 & 90.2 & 95.7 & 88.2 & 92.3 & 90.2 & 90.7 & 93.3 & 92.0  \\
\bottomrule
\end{tabular}}
\label{tab:voc}
\end{table*}
%  83.3 & 75.0 & 78.5 & 76.7 & 80.3 & 82.6 & 81.5 
% \rowcolor{gray!9} 
% \Xhline{5-8}{1.5pt}
% \cline{5-18}{\vrule width 1.5pt}
% \Xcline{5-18}{2pt}  % 加粗为 2pt
% \rowcolor{gray!9}
% \midrule
% \rowcolor{igray}
% \multirow{-1.8}{*}{\cellcolor{igray}Backbone} &  \cellcolor{igray}Prompt &  \cellcolor{igray}Group &  \cellcolor{igray}MoE &  mAP &  CP & CR & CF1 & OP & OR & OF1 &  mAP & CP & CR & CF1 & OP & OR & OF1 \\ 
% \midrule
% \Xcline{2pt}
% 
% \begin{table*}[hbt!]
% \begin{tabular}{c}
% \hline
% \noalign{\vskip -2pt}  % 调整线条位置
% \vrule height 2pt width \linewidth depth 0pt  % 自定义横线
% \noalign{\vskip 2pt}
% Data \\
% \hline
% \end{tabular}
% \end{table*}
% \begin{table*}
% \begin{tabular}{|>{\columncolor{gray!1}}c|>{\columncolor{gray!9}}c|>{\columncolor{gray!9}}c|}
% \hline
% \textbf{Header 1} & \textbf{Header 2} & \textbf{Header 3} \\ 
% \hline
% Data 1 & Data 2 & Data 3 \\
% \hline
% \end{tabular}
% \end{table*}
% \begin{table*}[hbt!]
% % \setlength{\tabcolsep}{5pt}
% % \setlength{\extrarowheight}{5pt} % 增加行高
% \centering
% \resizebox{\linewidth}{!}
% {\begin{tabular}{c|c c c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
% \hline\thickhline
% % \midrule
% % \rowcolor{igray}
% \multicolumn{1}{c|}{\cellcolor{igray}\multirow{2}{*}{Backbone}}  & 
% \multicolumn{3}{c|}{\cellcolor{igray}Scope} &
% % \cline{2-3}
% \multicolumn{7}{c|}{\cellcolor{igray}Resolution: 224 $\times$ 224} & \multicolumn{7}{c}{\cellcolor{igray}Resolution: 448 $\times$ 448} \\ 
% \cline{5-18}
% % \rowcolor{igray}
% \multicolumn{1}{l|}{\cellcolor{igray}} & \cellcolor{igray} Prompt & \cellcolor{igray} Group & \cellcolor{igray} MoE & \cellcolor{igray} mAP &  \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 & \cellcolor{igray} mAP & \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 \\ 
% \midrule
% \midrule
% ViT-B          & 1 & 2 &  3 &  4   &  5   &  6   &  7   &  8   &  9  & 10 &  11 &  12  & 13 & 14 & 15 & 16 & 17 \\
% % SRN               & 224$\times$224 & 77.1 & 81.6 & 65.4 & 71.2 & 82.7 & 69.9 & 75.8 & 85.2 & 58.8 & 67.4 & 87.4 & 62.5 & 72.9\\
% % ResNet-101        & 224$\times$224 & 78.3 & 80.2 & 66.7 & 72.8 & 83.9 & 70.8 & 76.8 & 84.1 & 59.4 & 69.7 & 89.1 & 62.8 & 73.6\\
% \midrule
% \end{tabular}}
% \vspace{0.1cm}
% \caption{Comparison of our method with known state-of-the-art models on MS-COCO at medium input resolution. The backbones noted with 22k are pretrained on the ImageNet-22k dataset.
% Among them, mAP, OF1, and CF1 are the primary metrics (shaded in the table) as the others may be affected by the chosen threshold largely. All metrics are in \%.}
% \label{Table:coco}
% \end{table*}
% \begin{table*}[h]
% \begin{tabular}{|c|c|}
% \hline
% \cellcolor{blue!25}\textcolor{white}{data1} & \cellcolor{blue!25}\textcolor{white}{data2} \\
% \hline
% data3 & data4 \\
% \hline
% \end{tabular}
% \end{table*}
% \setlength{\tabcolsep}{5pt}
% \setlength{\arrayrulewidth}{1.5pt}
% \setlength{\extrarowheight}{5pt} % 增加行高
% \begin{table*}[!t]
% \centering
% \caption{Comparison of our method with known state-of-the-art models on MS-COCO at medium input resolution. The backbones noted with 22k are pre-trained on the ImageNet-22k dataset.
% Among them, mAP, OF1, and CF1 are the primary metrics (shaded in the table) as the others may be affected by the chosen threshold largely. All metrics are in \%.}
% \resizebox{\linewidth}{!}
% {\begin{tabular}{c|c c c c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
% \hline\thickhline
% \multicolumn{1}{c|}{\multirow{2}{*}{\cellcolor{igray}}}
% & 
% \multicolumn{4}{c|}{\cellcolor{igray}Scope} &
% \multicolumn{7}{c|}{\cellcolor{igray}Resolution: 224 $\times$ 224} & \multicolumn{7}{c}{\cellcolor{igray}Resolution: 448 $\times$ 448} \\ 
% \cline{6-19}
% \multirow{-1.8}{*}{\cellcolor{igray}Backbone} &  \cellcolor{igray}GateVPT~\cite{yoo2023improving} & \cellcolor{igray}VPT~\cite{jia2022visual} &  \cellcolor{igray}Group &  \cellcolor{igray}MoE &  \cellcolor{igray}mAP &  \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 &  \cellcolor{igray}mAP & \cellcolor{igray}CP & \cellcolor{igray}CR & \cellcolor{igray}CF1 & \cellcolor{igray}OP & \cellcolor{igray}OR & \cellcolor{igray}OF1 \\ 
% \hline
% \midrule
% ViT-B         & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% ViT-B         &            & \checkmark &            &            & 76.9 & 70.9 & 71.4 & 71.1 & 73.9 & 74.7 & 74.3 & - & - & - & -  & - & - & - \\
% ViT-B         &            &            & \checkmark &            & 78.4 & 72.0 & 72.6 & 72.3 & 75.0 & 75.7 & 75.3 & - & - & - & -  & - & - & - \\
% ViT-B         &            &            & \checkmark & \checkmark & 79.3 & 72.8 & 73.4 & 73.1 & 75.6 & 76.4 & 76.0 & - & - & - & -  & - & - & - \\
% \midrule
% MEA              & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% MEA              &            & \checkmark &            &            & 68.2 & 63.9 & 64.4 & 64.2 & 69.6 & 70.3 & 70.0 & - & - & - & -  & - & - & - \\
% MEA              &            &            & \checkmark &            & 71.2 & 66.1 & 66.6 & 66.4 & 71.5 & 72.3 & 71.9 & - & - & - & -  & - & - & - \\
% MEA              &            &            & \checkmark & \checkmark & 74.6 & 68.8 & 69.4 & 69.1 & 73.5 & 74.3 & 73.9 & - & - & - & -  & - & - & - \\
% \midrule
% MoCo v3           & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% MoCo v3           &            & \checkmark &            &            & 71.9 & 66.6 & 67.2 & 66.9 & 71.1 & 71.9 & 71.5 & - & - & - & -  & - & - & - \\
% MoCo v3           &            &            & \checkmark &            & 72.9 & 67.5 & 68.0 & 67.8 & 71.8 & 72.6 & 72.2 & - & - & - & -  & - & - & - \\
% MoCo v3           &            &            & \checkmark & \checkmark & 74.4 & 68.8 & 69.3 & 69.0 & 72.9 & 73.6 & 73.2 & - & - & - & -  & - & - & - \\
% \midrule
% ViT-B-21k     & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% ViT-B-21k     &            & \checkmark &            &            & 81.0 & 74.5 & 75.1 & 74.8 & 77.3 & 78.1 & 77.7 & - & - & - & -  & - & - & - \\
% ViT-B-21k     &            &            & \checkmark &            & 82.1 & 75.5 & 76.0 & 75.7 & 77.9 & 78.8 & 78.4 & - & - & - & -  & - & - & - \\
% ViT-B-21k     &            &            & \checkmark & \checkmark & 82.9 & 76.0 & 76.6 & 76.3 & 78.5 & 79.4 & 78.9 & - & - & - & -  & - & - & - \\
% \midrule
% DINOv2/B         & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% DINOv2/B         &            & \checkmark &            &            & 86.1 & 79.5 & 80.1 & 79.8 & 81.9 & 82.8 & 82.4 & - & - & - & -  & - & - & - \\
% DINOv2/B         &            &            & \checkmark &            & 87.0 & 80.3 & 80.9 & 80.6 & 82.7 & 83.5 & 83.1 & - & - & - & -  & - & - & - \\
% DINOv2/B         &            &            & \checkmark & \checkmark & 87.4 & 80.6 & 81.2 & 80.9 & 82.9 & 83.8 & 83.4 & - & - & - & -  & - & - & - \\
% \midrule
% DINOv2/S         & \checkmark &            &            &            & - & - & - & - & - & - & - & - & - & - & -  & - & - & - \\
% DINOv2/S         &            & \checkmark &            &            & 80.1 & 73.8 & 74.4 & 74.1 & 77.1 & 77.9 & 77.5 & - & - & - & -  & - & - & - \\
% DINOv2/S         &            &            & \checkmark &            & 81.5 & 74.9 & 75.5 & 75.2 & 78.2 & 79.1 & 78.6 & - & - & - & - & - & - & - \\
% DINOv2/S         &            &            & \checkmark & \checkmark & 82.9 & 76.2 & 76.8 & 76.5 & 79.2 & 80.0 & 79.6 & - & - & - & -  & - & - & - \\
% \bottomrule
% \end{tabular}}
% \label{Table:coco}
% \end{table*}
